READMem: Robust Embedding Association for a Diverse Memory in Unconstrained Video Object Segmentation

We present READMem (Robust Embedding Association for a Diverse Memory), a modular framework for semi-automatic video object segmentation (sVOS) methods designed to handle unconstrained videos. Contemporary sVOS works typically aggregate video frames in an ever-expanding memory, demanding high hardware resources for long-term applications. To mitigate memory requirements and prevent near object duplicates (caused by information of adjacent frames), previous methods introduce a hyper-parameter that controls the frequency of frames eligible to be stored. This parameter has to be adjusted according to concrete video properties (such as rapidity of appearance changes and video length) and does not generalize well. Instead, we integrate the embedding of a new frame into the memory only if it increases the diversity of the memory content. Furthermore, we propose a robust association of the embeddings stored in the memory with query embeddings during the update process. Our approach avoids the accumulation of redundant data, allowing us in return, to restrict the memory size and prevent extreme memory demands in long videos. We extend popular sVOS baselines with READMem, which previously showed limited performance on long videos. Our approach achieves competitive results on the Long-time Video dataset (LV1) while not hindering performance on short sequences. Our code is publicly available.

==> figures/Macro_for_figures.tex <==
% ---- Algebra
%\newcommand{\veccs}[1]{\ensuremath{\mathbf{#1}}}
%\newcommand{\veccsdos}[2]{\ensuremath{\mathbf{#1}_#2}}
%\newcommand{\veccstres}[3]{\ensuremath{\mathbf{#1}_#2^#3}}
%\newcommand{\mset}[1]{\ensuremath{\mathcal{#1}}}
%\newcommand{\mtensor}[1]{\ensuremath{\mathbf{#1}}}
%\newcommand{\Card}[1]{$\lvert #1 \rvert$}
%\newcommand{\Mod}[1]{\ (\mathrm{mod}\ #1)}


% --------------------------
% - Random Value Generator -
% --------------------------
\newcommand*{\NewNumbers}{\pgfmathsetmacro{\randomA}{random(0,100)}} % Generate value between 0 and 100


% ------------------------
% - Draw Title of Figure -
% ------------------------
\newcommand\figxtitle{}
\def\figxtitle[#1]{% Display the figure's title, #1-> Text
	\draw[anchor=west] (-0.3,0.5) node {\textbf{#1}};
}

\newcommand\figxtext{}
\def\figxtext[#1,#2][#3]{% Display the figure's title, #1-> Text
	\draw[anchor=west] (#1,#2) node {\textit{#3}};
}

% -------------------
% - Draw the Origin -
% -------------------
\newcommand\showxorigin{}
\def\showxorigin[#1,#2]{% Show origin, #1-> x_xoord, #2-> y_coord
	\filldraw [fill=lightgray,draw=lightgray](O) circle [radius=2pt];
	\draw[->,lightgray] (#1,#2) -- (#1+1,#2) node[midway,above] {$x$};
	\draw[->,lightgray] (#1,#2) -- (#1,#2-1) node[midway,left] {$y$};
}

% ------------------
% - Display a Grid -
% ------------------
\newcommand\grid{}
\def\grid[#1,#2,#3,#4](#5,#6,#7){% Show origin, #1-> x_xoord, #2-> y_coord, #3->W, #4->H, #5-> stepsize, #6->color, #7->strengh
\draw [step=#5, #7, color=#6!10!white] (#2,#1) grid (#1+#3,#2+#4);
}


% -------------------
% - Draw a Matrix A -
% -------------------
\newcommand\drawxMatrixA{}
\def\drawxMatrixA[#1,#2,#3,#4](#5,#6,#7){% Draw a matrix, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color, #6 transparance_A, #7 transparance_B
	% Outline
    \draw [very thick] (#1,#2) rectangle (#1+#3,#2+#4);
    % Color
	\filldraw [fill=#5!#6!white,draw=#5!#7!black] (#1,#2) rectangle (#1+#3,#2+#4);
	% Grid
	\draw [step=0.1, very thin, color=gray] (#1,#2) grid (#1+#3,#2+#4);
}


% ---------------------------------------------------------
% - Draw Underbrace for spatial dimensions cues version A -
% ---------------------------------------------------------
\newcommand\WidthHeightChannelsUnderbrance{}
\def\WidthHeightChannelsUnderbrance[#1,#2,#3,#4](#5,#6,#7)[#8]{ % Draw undevrances, #1-> x_start, #2-> y_start, #3-> width, #4-> height, #5-> width name, #6-> height name, #7-> channel name, #8-> size of the diagonal typically sqrt((#2+#3)^^2)/(#2+#3)
    \draw (#1+#3/2,#2-1.30) node {\scriptsize{\color{gray}#5}};
	\draw (#1+#3/2,#2-1.13) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	\draw (#1-0.31,#2-#4/2) node {\scriptsize{\color{gray}#6}};
	\draw (#1-0.13,#2-#4/2) node[rotate = 270] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
	\draw (#1+1.55,#2-1.00) node {\scriptsize{\color{gray}#7}};
	\draw (#1+1.35,#2-0.85) node[rotate = 45] {{\color{gray!65}$\underbrace{\hspace{#8cm}}$}};
}

% ---------------------------------------------------------
% - Draw Underbrace for spatial dimensions cues version B -
% ---------------------------------------------------------
\newcommand\WidthHeightUnderbrance{}
\def\WidthHeightUnderbrance[#1,#2,#3,#4](#5,#6){ % Draw undevrances, #1-> x_start, #2-> y_start, #3-> width, #4-> height, #5-> width name, #6-> height name
    \draw (#1+#3/2,#2-#4-0.30) node {\scriptsize{\color{gray}#5}};
	\draw (#1+#3/2,#2-#4-0.13) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	\draw (#1+#3 + 0.4,#2-#4/2-0.02) node {\scriptsize{\color{gray}#6}};
	\draw (#1+#3 + 0.13,#2-#4/2) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
}

\newcommand\WidthHeightUnderbranceForThreeLetters{}
\def\WidthHeightUnderbranceForThreeLetters[#1,#2,#3,#4](#5,#6){ % Draw undevrances, #1-> x_start, #2-> y_start, #3-> width, #4-> height, #5-> width name, #6-> height name
	\draw (#1+#3/2,#2-#4-0.30) node {\scriptsize{\color{gray}#5}};
	\draw (#1+#3/2,#2-#4-0.13) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	\draw (#1+#3 + 0.55,#2-#4/2) node {\scriptsize{\color{gray}#6}};
	\draw (#1+#3 + 0.13,#2-#4/2) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
}


% -----------------
% - Draw Equation -
% -----------------
\newcommand\WriteEq{}
\def\WriteEq[#1,#2](#3)[#4]{ % Draw an equation, #1-> x_start, #2-> y_start, #3-> color, #4-> Equation in math mode $eq$
	\draw[anchor=west] (#1,#2) node {\color{#3}\scriptsize{#4}};
}

% --------------------------------------------
% - Draw a collection A of simple Matrices A -
% --------------------------------------------
\newcommand\drawxColllectionOfMatrixA{}
\def\drawxColllectionOfMatrixA[#1,#2,#3,#4](#5){% Draw a collection of matrices, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color
	\drawxMatrixA[#1+0.7,#2-0.3,#3,-#4](#5,80,40)
	\drawxMatrixA[#1+0.6,#2-0.4,#3,-#4](#5,70,40)
	\drawxMatrixA[#1+0.5,#2-0.5,#3,-#4](#5,60,40)
	\drawxMatrixA[#1+0.4,#2-0.6,#3,-#4](#5,50,40)
	\drawxMatrixA[#1+0.3,#2-0.7,#3,-#4](#5,40,40)
	\drawxMatrixA[#1+0.2,#2-0.8,#3,-#4](#5,30,40)
}

% -------------------------------
% - Draw a complex of matrice A -
% -------------------------------
\newcommand\drawxComplexOfMatrixA{}
\def\drawxComplexOfMatrixA[#1,#2,#3,#4](#5)[#6]{% Draw a collection of matrices, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color, #6-> Equation in math mode $eq$ #6-> Eq
	\drawxColllectionOfMatrixA[#1,#2,#3,#4](#5)
	\WidthHeightChannelsUnderbrance[#1+0.2,#2-0.8,#3,#4]($w$,$h$,$c_k$)[0.7]
	\WriteEq[#1,#2-2.3](#5)[#6]
}


% -----------------
% - Draw an arrow -
% -----------------
\newcommand\drawxArrow{}
\def\drawxArrow[#1,#2,#3,#4](#5){% #1 x start, #2-> y start, #3-> w, #4-> h, #5-> Color
	\draw[->,#5] (#1,#2) -- (#1+#3,#2+#4);
}

\newcommand\drawxArrowTxt{}
\def\drawxArrowTxt[#1,#2,#3,#4](#5)[#6]{% #1 x start, #2-> y start, #3-> w, #4-> h, #5-> Color
	\draw[->,#5] (#1,#2) -- (#1+#3,#2+#4) node [midway,above,align=left] {#6};
}
\newcommand\drawxLine{}
\def\drawLine[#1,#2,#3,#4](#5){% #1 x start, #2-> y start, #3-> w, #4-> h, #5-> Color
	\draw[#5, thick] (#1,#2) -- (#1+#3,#2+#4);
}

% -------------
% - Draw Dots -
% -------------
\newcommand\drawdots{}
\def\drawdots[#1,#2,#3,#4](#5,#6){
	\draw[decorate sep={#5mm}{#6mm},fill] (#1,#2) -- (#1+#3,#2-#4);
}


% -------------------
% - Draw Matrices B -
% -------------------
\newcommand\drawxMatrixB{}
\def\drawxMatrixB[#1,#2,#3,#4](#5)[#6]{% Draw a collection of matrices, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color, #6 step
\draw [very thick] (#1,#2) rectangle (#1+#3,#2-#4);
\filldraw [fill=#5!80!white,draw=#5!40!black] (#1,#2-0*#6) rectangle (#1+#3,#2-1*#6);
\filldraw [fill=#5!70!white,draw=#5!40!black] (#1,#2-1*#6) rectangle (#1+#3,#2-2*#6);
\filldraw [fill=#5!60!white,draw=#5!40!black] (#1,#2-2*#6) rectangle (#1+#3,#2-3*#6);
\filldraw [fill=#5!50!white,draw=#5!40!black] (#1,#2-3*#6) rectangle (#1+#3,#2-4*#6);
\filldraw [fill=#5!40!white,draw=#5!40!black] (#1,#2-4*#6) rectangle (#1+#3,#2-5*#6);
\filldraw [fill=#5!30!white,draw=#5!40!black] (#1,#2-5*#6) rectangle (#1+#3,#2-6*#6);
\draw [step=#6, very thin, color=gray] (#1,#2) grid (#1+#3,#2-#4);
}

% -------------------
% - Draw Transpose Matrices B -
% -------------------
\newcommand\drawxTransposeMatrixB{}
\def\drawxTransposeMatrix[#1,#2,#3,#4](#5)[#6]{% Draw a collection of matrices, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color, #6 step
	\draw [very thick] (#1,#2) rectangle (#1+#4,#2-#3);
	\filldraw [fill=#5!80!white,draw=#5!40!black] (#1+0*#6,#2) rectangle (#1+1*#6,#2-#3);
	\filldraw [fill=#5!70!white,draw=#5!40!black] (#1+1*#6,#2) rectangle (#1+2*#6,#2-#3);
	\filldraw [fill=#5!60!white,draw=#5!40!black] (#1+2*#6,#2) rectangle (#1+3*#6,#2-#3);
	\filldraw [fill=#5!50!white,draw=#5!40!black] (#1+3*#6,#2) rectangle (#1+4*#6,#2-#3);
	\filldraw [fill=#5!40!white,draw=#5!40!black] (#1+4*#6,#2) rectangle (#1+5*#6,#2-#3);
	\filldraw [fill=#5!30!white,draw=#5!40!black] (#1+5*#6,#2) rectangle (#1+6*#6,#2-#3);
	\draw [step=#6, very thin, color=gray] (#1,#2) grid (#1+#4,#2-#3);
}


\newcommand\drawxComplexOfMatrixB{}
\def\drawxComplexOfMatrixB[#1,#2,#3,#4](#5)[#6]{% Draw a collection of matrices, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color, #6-> Equation in math mode $eq$ #6-> Eq, #7-> step
    \drawxMatrixB[#1,#2,#3,#4](#5)[0.1]
	\WidthHeightUnderbrance[#1,#2,#3,#4]($hw$,$c_k$)
	\WriteEq[#1,#2-1.2](#5)[#6]
}

\newcommand\drawxComplexOfMatrixC{}
\def\drawxComplexOfMatrixC[#1,#2,#3,#4](#5){% Draw a collection of matrices, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color, #6-> Equation in math mode $eq$ #6-> Eq, #7-> step
	\drawxMatrixC[#1,#2,#3,#4](#5)[0.1]
	\WidthHeightUnderbrance[#1,#2,#3,#4]($hw$,$c_v$)
}

\newcommand\drawxMatrixC{}
\def\drawxMatrixC[#1,#2,#3,#4](#5)[#6]{% Draw a collection of matrices, #1-> x_start, #2-> y_start, #3-> width, #4->height, #5-> color, #6 step
	\draw [very thick] (#1,#2) rectangle (#1+#3,#2-#4);
	\filldraw [fill=#5!100!white,draw=#5!40!black] (#1,#2-0*#6) rectangle (#1+#3,#2-1*#6);
	\filldraw [fill=#5!90!white,draw=#5!40!black]  (#1,#2-1*#6) rectangle (#1+#3,#2-2*#6);
	\filldraw [fill=#5!80!white,draw=#5!40!black]  (#1,#2-2*#6) rectangle (#1+#3,#2-3*#6);
	\filldraw [fill=#5!70!white,draw=#5!40!black]  (#1,#2-3*#6) rectangle (#1+#3,#2-4*#6);
	\filldraw [fill=#5!60!white,draw=#5!40!black]  (#1,#2-4*#6) rectangle (#1+#3,#2-5*#6);
	\filldraw [fill=#5!50!white,draw=#5!40!black]  (#1,#2-5*#6) rectangle (#1+#3,#2-6*#6);
	\filldraw [fill=#5!40!white,draw=#5!40!black]  (#1,#2-6*#6) rectangle (#1+#3,#2-7*#6);
	\filldraw [fill=#5!30!white,draw=#5!40!black]  (#1,#2-7*#6) rectangle (#1+#3,#2-8*#6);
	\filldraw [fill=#5!20!white,draw=#5!40!black]  (#1,#2-8*#6) rectangle (#1+#3,#2-9*#6);
	\filldraw [fill=#5!10!white,draw=#5!40!black]  (#1,#2-9*#6) rectangle (#1+#3,#2-10*#6);
	\draw [step=#6, very thin, color=gray] (#1,#2) grid (#1+#3,#2-#4);
}


\newcommand\drawxCollectionOfMatrixBStackVertical{}
\def\drawxCollectionOfMatrixBStackVertical[#1,#2,#3,#4](#5)[#6]{
	\drawxTransposeMatrix[#1,#2-0*#3,#3,#4](#5)[#6]
	\drawxTransposeMatrix[#1,#2-1*#3,#3,#4](#5)[#6]
	\drawxTransposeMatrix[#1,#2-2*#3,#3,#4](#5)[#6]
}

\newcommand\drawxComplexOfMatrixBStackVertical{}
\def\drawxComplexOfMatrixBStackVertical[#1,#2,#3,#4](#5)[#6]{
\drawxCollectionOfMatrixBStackVertical[#1,#2,#3,#4](#5)[#6]
\WidthHeightUnderbranceForThreeLetters[#1,#2,#4,6]($c_k$,$nhw$)
}

\newcommand\drawAffinityMatrix{}
\def\drawAffinityMatrix[#1,#2,#3,#4][#5](#6,#7){% #1x,#2,#3w,#4h,#5step,#6math experssion for w,#7 math expression for h
	\draw [very thick] (#1,#2-0*#4) rectangle (#1+#3,#2-1*#4);
	\drawAffinityMatrixBlack[#1,#2-0*#4,#3,#4][#5](Black,1)
	%\draw [step=#5, very thin, color=gray] (#1,#2-0*#4) grid (#1+#3,#2-1*#4);
	\draw [very thick] (#1,#2-1*#4) rectangle (#1+#3,#2-2*#4);
	\drawAffinityMatrixBlack[#1,#2-1*#4,#3,#4][#5](Black,2)
%	\draw [step=#5, very thin, color=gray] (#1,#2-1*#4) grid (#1+#3,#2-2*#4);
	\draw [very thick] (#1,#2-2*#4) rectangle (#1+#3,#2-3*#4);	
	\drawAffinityMatrixBlack[#1,#2-2*#4,#3,#4][#5](Black,3)
%	\draw [step=#5, very thin, color=gray] (#1,#2-2*#4) grid (#1+#3,#2-3*#4);
	\WidthHeightUnderbranceForThreeLetters[#1,#2,#4,6](#6,#7)
}


\newcommand\drawAffinityMatrixSplit{}
\def\drawAffinityMatrixSplit[#1,#2,#3,#4][#5]{%(#6,#7){% #1x,#2,#3w,#4h,#5step,#6math experssion for w,#7 math expression for h
	\def\offsety{0.6}
	
	\draw [anchor=west](#1-0.3,#2+0.2) node {{\color{black}\scriptsize{$i=1$}}};
	\draw [very thick] (#1,#2-0*#4) rectangle (#1+#3,#2-1*#4);
	\drawAffinityMatrixBlack[#1,#2-0*#4,#3,#4][#5](Black,1)
	%\draw [step=#5, very thin, color=gray] (#1,#2-0*#4) grid (#1+#3,#2-1*#4);
	\draw (#1+#3 + 0.45,#2-#4/2) node {\scriptsize{\color{LimeGreen}$hw$}};
	\draw (#1+#3 + 0.13,#2-#4/2) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
	\draw (#1+#3/2,#2-#4-0.30) node {\scriptsize{\color{Red}$hw$}};
	\draw (#1+#3/2,#2-#4-0.13) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	
	\draw [anchor=west](#1-0.3,#2-1*#4-\offsety+0.2) node {{\color{black}\scriptsize{$i=2$}}};
	\draw [very thick] (#1,#2-1*#4-\offsety) rectangle (#1+#3,#2-2*#4-\offsety);
	\drawAffinityMatrixBlack[#1,#2-1*#4-\offsety,#3,#4][#5](Black,2)
%	\draw [step=#5, very thin, color=gray] (#1,#2-1*#4-\offsety) grid (#1+#3,#2-2*#4-\offsety);
	\draw (#1+#3 + 0.45,#2-1*#4-#4/2-\offsety) node {\scriptsize{\color{LimeGreen}$hw$}};
	\draw (#1+#3 + 0.13,#2-1*#4-#4/2-\offsety) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
	\draw (#1+#3/2,#2-2*#4-0.3-\offsety) node {\scriptsize{\color{Red}$hw$}};
	\draw (#1+#3/2,#2-2*#4-0.13-\offsety) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	
	\drawdots[#1+#3/2,#2-2*#4-1.2,0,0.6](1,3)
	
	\def\offsetyy{1.5}
	
	\draw [anchor=west](#1-0.3,#2-2*#4-\offsety+0.2-\offsetyy) node {{\color{black}\scriptsize{$i=n$}}};
	\draw [very thick] (#1,#2-2*#4-\offsety-\offsetyy) rectangle (#1+#3,#2-3*#4-\offsety-\offsetyy);
	\drawAffinityMatrixBlack[#1,#2-2*#4-\offsety-\offsetyy,#3,#4][#5](Black,3)
%	\draw [step=#5, very thin, color=gray] (#1,#2-2*#4-\offsety-\offsetyy) grid (#1+#3,#2-3*#4-\offsety-\offsetyy);
	\draw (#1+#3 + 0.45,#2-2*#4-#4/2-\offsety-\offsetyy) node {\scriptsize{\color{LimeGreen}$hw$}};
	\draw (#1+#3 + 0.13,#2-2*#4-#4/2-\offsety-\offsetyy) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
	\draw (#1+#3/2,#2-3*#4-0.3-\offsety-\offsetyy) node {\scriptsize{\color{Red}$hw$}};
	\draw (#1+#3/2,#2-3*#4-0.13-\offsety-\offsetyy) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	
}

\newcommand\drawAffinityMatrixOne{}
\def\drawAffinityMatrixOne[#1,#2,#3,#4][#5](#6,#7){%#1->Ox,#2->Oy,#3->w,#4->h,#5->step, #6-> color
	\draw [very thick] (#1,#2-0*#4) rectangle (#1+#3,#2-1*#4);
	\draw [step=#5, very thin, color=gray] (#1,#2-0*#4) grid (#1+#3,#2-1*#4);
	\draw (#1+#3 + 0.45,#2-#4/2) node {\scriptsize{\color{LimeGreen}$hw$}};
	\draw (#1+#3 + 0.13,#2-#4/2) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
	\draw (#1+#3/2,#2-#4-0.30) node {\scriptsize{\color{Red}$hw$}};
	\draw (#1+#3/2,#2-#4-0.13) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	
	% Generate a random value	
	\pgfmathsetseed{1}
	
	\drawAffinityMatrixBlack[#1,#2,#3,#4][#5](#6,#7)
}


\newcommand\drawAffinityMatrixBlack{}
\def\drawAffinityMatrixBlack[#1,#2,#3,#4][#5](#6,#7){%#1->Ox,#2->Oy,#3->w,#4->h,#5->step, #6-> color, #7->randomseed
	\pgfmathsetseed{#7}
	\foreach \idx in {0,...,19}{
		\foreach \jdx in {0,...,19}{
			%\def\randomxA{int(random(0,100)}
			\NewNumbers
			\filldraw[fill=#6!\randomA!white,draw=Red!40!black, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
		}
	} 
}

\newcommand\drawAffinityMatrixFinal{}
\def\drawAffinityMatrixFinal[#1,#2,#3,#4][#5]{%#1->Ox,#2->Oy,#3->w,#4->h
	\gdef\vlist{}
	\gdef\ilist{}
	\gdef\jlist{}
	\foreach \idx in {0,...,57}{
		\foreach \jdx in {0,...,19}{
			\xdef\jlist{\jlist, \jdx}
			\xdef\ilist{\ilist, \idx}
		}
	}

	\pgfmathparse{\mylist[3]}\pgfmathresult
%	\draw (#1+0.1*\jdx,#2) node {\ilist};
%	\draw (#1+0.1*\jdx,#2-0,5) node {\jlist};
%	\draw (#1+0.1*\jdx,#2) node {\ilist[0]};
%	\draw (#1+0.1*\jdx,#2-0,5) node {\jlist[0]};
	\gdef\vlist{}
	\gdef\ilist{}
	\gdef\jlist{}
}
%	\foreach \idx in {0,...,19}
%		\foreach \jdx in {0,...,19}{
%			%\def\randomxA{int(random(0,100)}
%			\NewNumbers
%			\filldraw[fill=#6!\randomA!white,draw=Red!40!black, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
%	
%	\foreach \i in {1,2,3} {
%		\xdef\alist{\alist \i/1,}
%		\xdef\vlist{\vlist \i/1,}
%	}
%
%		\ifnum \randomA > 60
%\filldraw[fill=#6!\randomA!white,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
%\else
%\filldraw[fill=white,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
%\fi


%	\xdef\vlist{\vlist 4/1}
%%	\pgfmathsetseed{#7}
%	

	
	
	
	
	

\newcommand\drawechellecouleur{}
\def\drawechellecouleur[#1,#2,#3,#4][#5](#6){%#1->Ox,#2->Oy,#3->w,#4->h,#5->step, #6-> color
	\draw [top color=#6, bottom color=white, draw=Red!40!black, very thin] (#1,#2) rectangle (#1+#3,#2-#4);
}

\newcommand\drawScatterMatrix{}
\def\drawScatterMatrix[#1,#2,#3,#4][#5](#6,#7)[#8]{% #1x,#2,#3w,#4h,#5step,#6math experssion for w,#7 math expression for h,#8 color
	\draw [very thick] (#1,#2-0*#4) rectangle (#1+#3,#2-1*#4);
	\drawScatterMatrixOrange[#1,#2-0*#4,#3,#4][#5](#8,1)
	\draw [step=#5, very thin, color=gray] (#1,#2-0*#4) grid (#1+#3,#2-1*#4);
	\draw [very thick] (#1,#2-1*#4) rectangle (#1+#3,#2-2*#4);
	\drawScatterMatrixOrange[#1,#2-1*#4,#3,#4][#5](#8,2)
	\draw [step=#5, very thin, color=gray] (#1,#2-1*#4) grid (#1+#3,#2-2*#4);
	\draw [very thick] (#1,#2-2*#4) rectangle (#1+#3,#2-3*#4);	
	\drawScatterMatrixOrange[#1,#2-2*#4,#3,#4][#5](#8,3)
	\draw [step=#5, very thin, color=gray] (#1,#2-2*#4) grid (#1+#3,#2-3*#4);
	\WidthHeightUnderbranceForThreeLetters[#1,#2,#4,6](#6,#7)
}

\newcommand\drawScatterMatrixOrange{}
\def\drawScatterMatrixOrange[#1,#2,#3,#4][#5](#6,#7){%#1->Ox,#2->Oy,#3->w,#4->h,#5->step, #6-> color, #7->randomseed
	\pgfmathsetseed{#7}
	\foreach \idx in {0,...,19}
	\foreach \jdx in {0,...,19}{
		%\def\randomxA{int(random(0,100)}
		\NewNumbers
		\ifnum \randomA > 60
			\filldraw[fill=#6!\randomA!white,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
		\else
			\filldraw[fill=white,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
		\fi
	} 
}

\newcommand\drawArgMaxMatrix{}
\def\drawArgMaxMatrix[#1,#2,#3,#4][#5](#6,#7){%#1->Ox,#2->Oy,#3->w,#4->h,#5->step, #6-> color, #7->randomseed
	\pgfmathsetseed{#7}
	\draw [very thick] (#1,#2-0*#4) rectangle (#1+#3,#2-1*#4);
	\foreach \idx in {0,...,19}{
		\foreach \jdx in {0,...,19}{
			%\def\randomxA{int(random(0,100)}
			\NewNumbers
			\ifnum \randomA > 95
			\filldraw[fill=#6,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
			\else
			\filldraw[fill=white,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
			\fi
		}
	}
	\draw [step=#5, very thin, color=gray] (#1,#2-0*#4) grid (#1+#3,#2-1*#4);
	\draw (#1+#3 + 0.45,#2-#4/2) node {\scriptsize{\color{LimeGreen}$hw$}};
	\draw (#1+#3 + 0.13,#2-#4/2) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
	\draw (#1+#3/2,#2-#4-0.30) node {\scriptsize{\color{Red}$hw$}};
	\draw (#1+#3/2,#2-#4-0.13) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
	
}

\newcommand\drawArgMaxMatrixTranspose{}
\def\drawArgMaxMatrixTranspose[#1,#2,#3,#4][#5](#6,#7){%#1->Ox,#2->Oy,#3->w,#4->h,#5->step, #6-> color, #7->randomseed
	\pgfmathsetseed{#7}
	\draw [very thick] (#1,#2-0*#4) rectangle (#1+#3,#2-1*#4);
	\foreach \jdx in {0,...,19}{
		\foreach \idx in {0,...,19}{
			%\def\randomxA{int(random(0,100)}
			\NewNumbers
			\ifnum \randomA > 95
			\filldraw[fill=#6,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
			\else
			\filldraw[fill=white,draw=white, very thin] (#1+\idx*#5,#2-\jdx*#5) rectangle (#1+\idx*#5+#5,#2-\jdx*#5-#5);
			\fi
		}
	}
	\draw [step=#5, very thin, color=gray] (#1,#2-0*#4) grid (#1+#3,#2-1*#4);
}


\newcommand\drawScatterMatrixSplit{}
\def\drawScatterMatrixSplit[#1,#2,#3,#4][#5]{%(#6,#7){% #1x,#2,#3w,#4h,#5step,#6math experssion for w,#7 math expression for h
		\def\offsety{0.6}
		
		\draw [anchor=west](#1-0.3,#2+0.2) node {{\color{black}\scriptsize{$i=1$}}};
		\draw [very thick] (#1,#2-0*#4) rectangle (#1+#3,#2-1*#4);
		\drawScatterMatrixOrange[#1,#2-0*#4,#3,#4][#5](teal,1)
		\draw [step=#5, very thin, color=gray] (#1,#2-0*#4) grid (#1+#3,#2-1*#4);
		\draw (#1+#3 + 0.45,#2-#4/2) node {\scriptsize{\color{LimeGreen}$hw$}};
		\draw (#1+#3 + 0.13,#2-#4/2) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
		\draw (#1+#3/2,#2-#4-0.30) node {\scriptsize{\color{Red}$hw$}};
		\draw (#1+#3/2,#2-#4-0.13) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
		
		\draw [anchor=west](#1-0.3,#2-1*#4-\offsety+0.2) node {{\color{black}\scriptsize{$i=2$}}};
		\draw [very thick] (#1,#2-1*#4-\offsety) rectangle (#1+#3,#2-2*#4-\offsety);
		\drawScatterMatrixOrange[#1,#2-1*#4-\offsety,#3,#4][#5](teal,2)
		\draw [step=#5, very thin, color=gray] (#1,#2-1*#4-\offsety) grid (#1+#3,#2-2*#4-\offsety);
		\draw (#1+#3 + 0.45,#2-1*#4-#4/2-\offsety) node {\scriptsize{\color{LimeGreen}$hw$}};
		\draw (#1+#3 + 0.13,#2-1*#4-#4/2-\offsety) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
		\draw (#1+#3/2,#2-2*#4-0.3-\offsety) node {\scriptsize{\color{Red}$hw$}};
		\draw (#1+#3/2,#2-2*#4-0.13-\offsety) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
		
		\drawdots[#1+#3/2,#2-2*#4-1.2,0,0.6](1,3)
		
		\def\offsetyy{1.5}
		
		\draw [anchor=west](#1-0.3,#2-2*#4-\offsety+0.2-\offsetyy) node {{\color{black}\scriptsize{$i=n$}}};
		\draw [very thick] (#1,#2-2*#4-\offsety-\offsetyy) rectangle (#1+#3,#2-3*#4-\offsety-\offsetyy);
		\drawScatterMatrixOrange[#1,#2-2*#4-\offsety-\offsetyy,#3,#4][#5](teal,3)
		\draw [step=#5, very thin, color=gray] (#1,#2-2*#4-\offsety-\offsetyy) grid (#1+#3,#2-3*#4-\offsety-\offsetyy);
		\draw (#1+#3 + 0.45,#2-2*#4-#4/2-\offsety-\offsetyy) node {\scriptsize{\color{LimeGreen}$hw$}};
		\draw (#1+#3 + 0.13,#2-2*#4-#4/2-\offsety-\offsetyy) node[rotate = 90] {{\color{gray!65}$\underbrace{\hspace{#4cm}}$}};
		\draw (#1+#3/2,#2-3*#4-0.3-\offsety-\offsetyy) node {\scriptsize{\color{Red}$hw$}};
		\draw (#1+#3/2,#2-3*#4-0.13-\offsety-\offsetyy) node[rotate = 0] {{\color{gray!65}$\underbrace{\hspace{#3cm}}$}};
		
	}

